Generating Informative Conclusions for Argumentative Texts

The purpose of an argumentative text is to support a certain conclusion. Yet, they are often omitted, expecting readers to infer them rather. While appropriate when reading an individual text, this rhetorical device limits accessibility when browsing many texts (e.g., on a search engine or on social media). In these scenarios, an explicit conclusion makes for a good candidate summary of an argumentative text. This is especially true if the conclusion is informative, emphasizing specific concepts from the text. With this paper we introduce the task of generating informative conclusions: First, Webis-ConcluGen-21 is compiled, a large-scale corpus of 136,996 samples of argumentative texts and their conclusions. Second, two paradigms for conclusion generation are investigated; one extractive, the other abstractive in nature. The latter exploits argumentative knowledge that augment the data via control codes and finetuning the BART model on several subsets of the corpus. Third, insights are provided into the suitability of our corpus for the task, the differences between the two generation paradigms, the trade-off between informativeness and conciseness, and the impact of encoding argumentative knowledge. The corpus, code, and the trained models are publicly available.

==> table-internal-evaluation.tex <==
\begin{table*}[tb]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\bfseries{Model} & \multicolumn{4}{c}{\bfseries{Automatic Evaluation}} & \multicolumn{5}{c}{\bfseries{Manual Evaluation}} \\ \midrule & \multicolumn{3}{@{}c@{\hspace{3\tabcolsep}}} {\bfseries Lexical} & \multicolumn{1}{l}{\bfseries Semantic}  & \multicolumn{2}{c}{\bfseries Is Conclusion} & \multicolumn{3}{c}{\bfseries Error Type}\\
\cmidrule(r{2\tabcolsep}){2-5}\cmidrule(r{1\tabcolsep}){6-7}\cmidrule(r{2\tabcolsep}){8-10}
& \multicolumn{1}{l}{\bfseries ROUGE-1} & \multicolumn{1}{l}{\bfseries ROUGE-2} & \multicolumn{1}{l}{\bfseries ROUGE-L} & \multicolumn{1}{l}

{\bfseries BERTScore} & \multicolumn{1}{c}{\bfseries \% Yes} & \multicolumn{1}{c}{\bfseries \% No} & \multicolumn{1}{l}{\bfseries \% Target} & \multicolumn{1}{l}{\bfseries \% Stance} & \multicolumn{1}{l}{\bfseries \% Non-Arg.} \\
\midrule
{\bfseries Abstractive} & & & & & & & & & \\
{\small\tt{dbart-XSum}}        & 18.2                        & 6.3                         & 16.2                        & 0.24                          & 20.9                      & 79.1                     & \phantom{0}9.1                        & 3.7                        & 66.3                            \\
{\small\tt{dbart-CMV}}         & 27.5                        & 13.8\phantom{0}             & 26.6                        & 0.38                          &  62\phantom{0.}           & 38\phantom{0.}           & 29.4                                  & 7.5                        & \phantom{0}0.1                  \\
{\small\tt{dbart-Debates}}     & 16\phantom{0.}              & 4.6                         & 15.1                        & 0.22                          & 25.7                      & 74.3                     & 50.8                                  & 5.9                        & 17.6                            \\
{\small\tt{dbart}}         & 29.8                        & 16.4\phantom{0}             & 29.3                        & 0.39                          & 69.5                      & 30.5                     & 21.4                                  & 5.4                        & \phantom{0}3.7                  \\
{\small\tt{dbart-Topic}}       & 26.6                        & 13\phantom{00.}             & 25.9                        & 0.36                          & 64.2                      & 35.8                     & 28.9                                  & 4.8                        & \phantom{0}2.1                  \\
{\small\tt{dbart-Aspects}}     & 29.6                        & 15\phantom{00.}             & 28.5                        & 0.39                          & 76.5                      & 23.5                     & 17.1                                  & 4.8                        & \phantom{0}1.6                  \\
{\small\tt{dbart-Targets}}     & 26.5                        & 12.2\phantom{0}             & 25.5                        & 0.36                          & 72.7                      & 27.3                     & 19.8                                  & 5.3                        & \phantom{0}2.2                  \\
\\
{\bfseries Extractive} & & & & & & & & & \\
{\small\tt{First-Sentence}}    & 14.6                        & 5.5                         & 13.6                        & 0.14                          & 25.7                      & 74.3                     & \phantom{0}7.5                        & -                          & 66.8                            \\
{\small\tt{Arg-PageRank}}      & 13.8                        & 4.6                         & 12.5                        & 0.16                          & 40.1                      & 59.9                     & 15.5                                  & -                          & 44.4                            \\
{\small\tt{Claim-Detection}}   & 13.4                        & 4.3                         & 12.5                        & 0.17                          & 32.1                      & 67.9                     & 28.9                                  & -                          & 39\phantom{0.}                  \\
\bottomrule
\end{tabular}
\caption{Automatic and manual evaluation on the internal test set of 187 (\emph{argumentative text, conclusion}) pairs. For BERTScore, we report the rescaled F-1 score. For manual evaluation, we show the percentage of conclusions generated and the percentage distribution of three error types among the non-conclusions. }
\label{table-internal-evaluation}
\end{table*}
